Private Federated Learning with Domain Adaptation

Federated Learning (FL) is a distributed machine learning (ML) paradigm that enables multiple parties to jointly re-train a shared model without sharing their data with any other parties, offering advantages in both scale and privacy. We propose a framework to augment this collaborative model-building with per-user domain adaptation. We show that this technique improves model accuracy for all users, using both real and synthetic data, and that this improvement is much more pronounced when differential privacy bounds are imposed on the FL model.

==> outline.tex <==

* Abstract

* Introduction:
    * Privacy preservation becoming increasingly foundational, but existing techniques
        lead to loss in accuracy.
    * Federated learning getting huge traction in academia and industry.
    * Domain adaptation important (with use cases [I'll need references here]).
    * Existing work on all these fields in ML does not put these together, which we do
        in this paper.  Need to cite recent transfer learning related work and contrast with our work.
    * Brief overview of proposed system and performance (accuracy) improvement claims.

* Background
    * Privacy in ML in more detail, describing differential privacy and PATE.  We focus on differential
        privacy, but our work applies to PATE as well.
    * Description on Federated Learning, and recent work on combining it with differential privacy.
    * Domain adaption description and its history (need references here).

* Our Approach
    * Bring together differentially private federated learning and domain adaptation.
    * Description of the system architecture (with picture?).

* Evaluation
    * I don't have any insights into how to write this.

